PROZE: Generating Parameterized Unit Tests Informed by Runtime Data

Typically, a conventional unit test (CUT) verifies the expected behavior of the unit under test through one specific input / output pair. In contrast, a parameterized unit test (PUT) receives a set of inputs as arguments, and contains assertions that are expected to hold true for all these inputs. PUTs increase test quality, as they assess correctness on a broad scope of inputs and behaviors. However, defining assertions over a set of inputs is a hard task for developers, which limits the adoption of PUTs in practice. In this paper, we address the problem of finding oracles for PUTs that hold over multiple inputs. We design a system called PROZE, that generates PUTs by identifying developer-written assertions that are valid for more than one test input. We implement our approach as a two-step methodology: first, at runtime, we collect inputs for a target method that is invoked within a CUT; next, we isolate the valid assertions of the CUT to be used within a PUT. We evaluate our approach against 5 real-world Java modules, and collect valid inputs for 128 target methods from test and field executions. We generate 2,287 PUTs, which invoke the target methods with a significantly larger number of test inputs than the original CUTs. We execute the PUTs and find 217 that provably demonstrate that their oracles hold for a larger range of inputs than envisioned by the developers. From a testing theory perspective, our results show that developers express assertions within CUTs that are general enough to hold beyond one particular input.

==> listings/rq2-put-1.tex <==
\begin{lstlisting}[style=java, showlines=true, label={lst:rq2-put-1}, caption={Excerpt from \texttt{testBagManagement\_PUT\_1}, containing the first assertion of the CUT \texttt{testBagManagement} of \autoref{lst:rq2-cut-put}. It is \greyassertion with the original argument of \texttt{createText}.}, firstnumber=42, float]
  ...
  assertEquals(value1, values.get(0));
  schem.removeUnqualifiedBagValue(bagName, value1);
  List<String> values2 = schem.getUnqualifiedBagValueList(bagName);
}
\end{lstlisting}


==> listings/rq2-put-2.tex <==
\begin{lstlisting}[style=java, showlines=true, label={lst:rq2-put-2}, caption={Excerpt from \texttt{testBagManagement\_PUT\_2}, containing the second assertion of the CUT \texttt{testBagManagement} of \autoref{lst:rq2-cut-put}. It is \greenassertion from the arguments of \texttt{createText}.}, firstnumber=42, float]
  ...
  assertEquals(value2, values.get(1));
  schem.removeUnqualifiedBagValue(bagName, value1);
  List<String> values2 = schem.getUnqualifiedBagValueList(bagName);
}
\end{lstlisting}


==> listings/rq2-put-3.tex <==
\begin{lstlisting}[style=java, showlines=true, label={lst:rq2-put-3}, caption={Excerpt from \texttt{testBagManagement\_PUT\_3}, containing the third assertion of the CUT \texttt{testBagManagement} of \autoref{lst:rq2-cut-put}. It is \greyassertion with the original argument of \texttt{createText}.}, firstnumber=42, float]
  ...
  schem.removeUnqualifiedBagValue(bagName, value1);
  List<String> values2 = schem.getUnqualifiedBagValueList(bagName);
  assertEquals(1, values2.size());
}
\end{lstlisting}


==> listings/rq2-put-4.tex <==
\begin{lstlisting}[style=java, showlines=true, label={lst:rq2-put-4}, caption={Excerpt from \texttt{testBagManagement\_PUT\_4}, containing the fourth assertion of the CUT \texttt{testBagManagement} of \autoref{lst:rq2-cut-put}. It is \goldassertion with the arguments provided to \texttt{createText}.}, firstnumber=42, float]
  ...
  schem.removeUnqualifiedBagValue(bagName, value1);
  List<String> values2 = schem.getUnqualifiedBagValueList(bagName);
  assertEquals(value2, values2.get(0));
}
\end{lstlisting}

